Automatic Repair and Deadlock Detection for Parameterized Systems

We present an algorithm for the repair of parameterized systems. The repair problem is, for a given process implementation, to find a refinement such that a given safety property is satisfied by the resulting parameterized system, and deadlocks are avoided. Our algorithm uses a parameterized model checker to determine the correctness of candidate solutions and employs a constraint system to rule out candidates. We apply this algorithm on systems that can be represented as well-structured transition systems (WSTS), including disjunctive systems, pairwise rendezvous systems, and broadcast protocols. Moreover, we show that parameterized deadlock detection can be decided in EXPTIME for disjunctive systems, and that deadlock detection is in general undecidable for broadcast protocols.

==> MC_Alg.tex <==
\section{Model Checking Algorithm}\label{app:mc_alg}
We present our model checking algorithm which is a variant of the known backwards reachability 
algorithm for WSTS~\cite{abdulla1996general}. We present it in detail to show how it stores intermediate results to return an \emph{error sequence}, from which we derive concrete error paths. 

\begin{algorithm}[h]
	\caption{Parameterized Model Checking}\label{alg:ParamMC}
	
	\begin{algorithmic}[1]		
		\Procedure{ModelCheck}{\emph{Counter System} $M$,$ERR$}
		\State $tempSet \gets ERR$, $E_0 \gets ERR$,
		$i \gets 1$, $visited \gets \emptyset$ \label{line:mc-initialise}
		{\color{brown}// A fixed point is reached if $visited = tempSet$} 
		\While{$tempSet \neq visited$} \label{line:mc-while}
		\State $visited \gets tempSet$ \label{line:mc-update}
		\State $E_i \gets minBasis(pred({\uparrow}E_{i-1}))$ \label{line:mc-pred} \\
		{\color{brown} //$pred$ is computed as in the proof of Lemma~\ref{lemma:basis-pred}} 
		\If{$E_i \cap \cstateset_0 \neq \emptyset$}\label{line:mc-intersect} \ \ {\color{brown} //intersect with initial states?}
		\State \textbf{return} $False,\{E_0,\ldots,E_i \cap \cstateset_0\}$\label{line:mc-error-sets}
		\EndIf
		\State $tempSet \gets minBasis(visited \cup E_i)$ \label{line:mc-update-temp} 
		\State $i \gets i+1$ 
		\EndWhile
		\State \textbf{return} $True,\emptyset$	\label{line:mc-true}			
		\EndProcedure
	\end{algorithmic}	
\end{algorithm}

\smartpar{Properties of Algorithm~\ref{alg:ParamMC}.}
Correctness of the algorithm follows from the correctness of the algorithm by
Abdulla et al.~\cite{abdulla1996general}, and from Lemma~\ref{lemma:basis-pred}. 
Termination follows from the fact that a non-terminating run would produce an infinite minimal basis, 
which is impossible since a minimal basis is an antichain.
%The complexity of such algorithms, which effectively check coverability in a VASS, is known to be EXPSPACE-complete~\cite{Rackoff78,Lipton76}.
\sj{mention complexity here?}

%any infinite increasing
%sequence $\cstateset_1 \subseteq \cstateset_2 \subseteq \cstateset_3 \subseteq
%\ldots$ of upward-closed
%sets eventually stabilizes, i.e. $\exists i \in \Nat$ with $\cstateset_i =
%\cstateset_{i+1} =
%\cstateset_{i+2} =  \ldots$ (cp. Finkel and Schnoebelen~\cite{finkel2001well}).

%Moreover, note that due to the cutoff results for disjunctive
%systems~\cite{Emerson00, JS2018VMCAI} and the fact that our algorithm finds shortest error paths, any state on the error paths
%will have a number of processes smaller than the cutoff.
